Progressive Conditioned Scale-Shift Recalibration of Self-Attention for Online Test-time Adaptation

Online test-time adaptation aims to dynamically adjust a network model in real-time based on sequential input samples during the inference stage. In this work, we find that, when applying a transformer network model to a new target domain, the Query, Key, and Value features of its self-attention module often change significantly from those in the source domain, leading to substantial performance degradation of the transformer model. To address this important issue, we propose to develop a new approach to progressively recalibrate the self-attention at each layer using a local linear transform parameterized by conditioned scale and shift factors. We consider the online model adaptation from the source domain to the target domain as a progressive domain shift separation process. At each transformer network layer, we learn a Domain Separation Network to extract the domain shift feature, which is used to predict the scale and shift parameters for self-attention recalibration using a Factor Generator Network. These two lightweight networks are adapted online during inference. Experimental results on benchmark datasets demonstrate that the proposed progressive conditioned scale-shift recalibration (PCSR) method is able to significantly improve the online test-time domain adaptation performance by a large margin of up to 3.9\% in classification accuracy on the ImageNet-C dataset.

==> IEEEabrv.bib.tex <==
@STRING{ieee_J_Access = "IEEE Access"}
@STRING{ieee_J_Acoust_Speech_Signal_Proc = "IEEE Trans. Acoust., Speech, Signal Process."}
@STRING{ieee_J_Aeron_Elect_Sys = "IEEE Trans. Aerosp. Electron. Syst."}
@STRING{ieee_J_Commun = "IEEE Commun. Mag."}
@STRING{ieee_J_Commun_Lett = "IEEE Commun. Lett."}
@STRING{ieee_J_Comput = "IEEE Comput."}
@STRING{ieee_J_Comput_Intell_AI = "IEEE Comput. Intell. Mag."}
@STRING{ieee_J_Image_Proc = "IEEE Trans. Image Process."}
@STRING{ieee_J_Inf_Theory = "IEEE Trans. Inf. Theory"}
@STRING{ieee_J_PAMI = "IEEE Trans. Pattern Anal. Mach. Intell."}
@STRING{ieee_J_Signal_Proc = "IEEE Signal Process. Mag."}
@STRING{ieee_J_Speech_Audio_Proc = "IEEE Trans. Speech Audio Process."}
@STRING{ieee_J_Video_Tech = "IEEE Trans. Circuits Syst. Video Technol."}

